In-Context Learning for Robots: Methods and Applications

General-purpose robots must infer what a new task requires and translate that understanding into appropriate physical action. In-context learning (ICL) for robots supports this process by using demonstrations and interaction to direct existing competence with neural parameters held fixed during deployment. We organize this literature review around the interfaces connecting contextual evidence to execution, distinguishing four families: context-conditioned policies, geometric demonstration transfer, world-model-based control, and skill- and agent-based execution. Comparing these interfaces clarifies their transfer assumptions and the roles of training, correspondence, and memory in making context useful. Across manipulation and navigation, we examine how these mechanisms preserve taught requirements as objects, environments, and execution conditions change. This analysis links method design to evaluation practices that distinguish responsiveness to teaching, physical transfer, and benefits from retained experience. The resulting agenda connects compositional task acquisition and faithful transfer with physical recursive self-improvement, in which experience improves the ability to learn subsequent tasks.

==> tables/geometric-reference-summary.tex <==
\begin{table}[!tp]
\centering
\surveytable
\caption{Geometric references and execution operations. Staged systems combine reference types; per-study details appear in Tables~\ref{tab:geometric-transfer} and~\ref{tab:correspondence-interfaces}.}
\label{tab:geometric-references}
\begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}p{0.25\linewidth}>{\raggedright\arraybackslash}p{0.32\linewidth}Y@{}}
\toprule
\textbf{Reference design} & \textbf{Operation} & \textbf{Examples} \\
\midrule
Visual alignment & View alignment; tracking; replay & FlowControl~\citep{argus2020flowcontrol}; DOME~\citep{valassakis2022dome}; DINOBot~\citep{dipalo2023dinobot} \\
\addlinespace[2pt]
Object-relative motion & Pose alignment; trajectory transform & Pose-based OSIL~\citep{vitiello2023pose}; DITTO~\citep{heppert2024ditto}; MT3~\citep{dreczkowski2025mt3} \\
\addlinespace[2pt]
Functional correspondence & Part matching; contact transfer & MAGIC~\citep{liu2024magic}; FUNCTO~\citep{tang2025functo}; SemAnCorr~\citep{dong2026semancorr} \\
\addlinespace[2pt]
Staged coordination & Arm coordination; stage alignment & ODIL~\citep{wang2025odil}; ManiLong-Shot~\citep{chen2025manilong}; annotation-free OSIL~\citep{wichitwechkarn2025annotationfree} \\
\bottomrule
\end{tabularx}
\par\phantomsection\label{floatend:tab:geometric-references}
\end{table}

